A Systematic Performance Analysis of Deep Perceptual Loss Networks: Breaking Transfer Learning Conventions

In recent years, deep perceptual loss has been widely and successfully used to train machine learning models for many computer vision tasks, including image synthesis, segmentation, and autoencoding. Deep perceptual loss is a type of loss function for images that computes the error between two images as the distance between deep features extracted from a neural network. Most applications of the loss use pretrained networks called loss networks for deep feature extraction. However, despite increasingly widespread use, the effects of loss network implementation on the trained models have not been studied. This work rectifies this through a systematic evaluation of the effect of different pretrained loss networks on four different application areas. Specifically, the work evaluates 14 different pretrained architectures with four different feature extraction layers. The evaluation reveals that VGG networks without batch normalization have the best performance and that the choice of feature extraction layer is at least as important as the choice of architecture. The analysis also reveals that deep perceptual loss does not adhere to the transfer learning conventions that better ImageNet accuracy implies better downstream performance and that feature extraction from the later layers provides better performance.

==> acronym.tex <==
\begin{acronym}[Bash]
    % General
    \acro{AI}{Artificial Intelligence}
    \acro{RL}{Reinforcement Learning}
    \acro{MLP}{Multilayer Perceptron}
    \acro{ANN}{Artificial Neural Network}
    \acro{CNN}{Convolutional Neural Network}
\end{acronym}

\acrodefplural{CNN}[CNNs]{Convolutional Neural Networks}

==> sections/8_biographies.tex <==

%\newpage

%\vspace{11pt}



%\vspace{-33pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/gustav_100x125.jpg}}]{Gustav~Grund~Pihlgren}
received his M.S., degree in Computer Science and Engineering from Chalmers University of Technology, Sweden, in 2018 and his \phd{} degree in Machine Learning from Luleå University of Technology, Sweden, in 2023.
He currently works as a postdoctoral fellow at Umeå University, Sweden, where he researches explainable AI techniques while maintaining collaboration with the Machine Learning Group at Luleå University of Technology.
His research interest includes machine learning, artificial intelligence, deep learning, explainable AI, feature learning, similarity metrics, and ethical AI.
\end{IEEEbiography}


%\vspace{-32pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/konstantina_100x125.png}}]{Konstantina~Nikolaidou}
received her B.S. in Physics and M.S., in Information Technologies with specialization in Big Data and Artificial Intelligence degrees from the National and Kapodistrian University of Athens, Greece, in 2018 and 2020, respectively.
She is currently a \phd{} candidate in Machine Learning at Luleå University of Technology, Sweden, since 2020. 
Her \phd{} research focuses on document image analysis and handwriting generation, and her interests further include computer vision and generative models.
\end{IEEEbiography}


%\vspace{-32pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/prakash_100x125.png}}]{Prakash~Chandra~Chhipa} received B.S., degree in mathematics \& physics and M.S., degree in computer science and applications from Rajasthan University, India, in 2006 and 2009, respectively.
Currently, he is a \phd{} candidate at Luleå University of Technology, Sweden, where he works with representation learning to reduce human supervision in learning phenomena, focusing mainly on self-supervised learning. 
He has previously worked in industrial R\&D for a decade with Samsung Research and Arkray R\&D, where he commercialized products in visual media and medical device domains and produced several invention disclosures with dozens of international patents.
\end{IEEEbiography}


%\vspace{-32pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/Nosheen.jpeg}}]{Nosheen~Abid}
received her M.S., degree in Computer Science with a specialization in machine learning and Natural Language Processing from the National University of Sciences and Technology, Pakistan, in 2018. She is currently doing a \phd{} in unsupervised deep learning approaches, mainly focusing on remote sensing and Earth Observation data from Lulea University of Technology, Sweden. She has obtained considerable theoretical and practical knowledge by working on machine learning and deep learning solutions in other disciplines like image enhancement, classification and segmentation, Natural Language Processing, FMRI images, sequential data, chatbots, and document analysis during my fellowships (DAAD in Germany, JICA in Japan) with the world's renowned AI institutes.
\end{IEEEbiography}


%\vspace{-32pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/rajkumar_100x125.png}}]{Rajkumar~Saini}
received his M.S., degree in computer science and engineering from Kamla Nehru Institute of Technology, India in 2014 and his \phd{} degree in machine learning from Indian Institute of Technology, Roorkee, India in 2019.
He is currently working as senior lecturer and researcher in the EISLAB Machine Learning, Luleå University of Technology, Sweden.
His research interests include computer vision, machine learning, pattern recognition, human-computer interaction, brain signal analysis, brain-computer interfaces, and digital image processing.
\end{IEEEbiography}


%\vspace{-32pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/fredrik_100x125.png}}]{Fredrik~Sandin}
received his M.S. degree in Engineering Physics at Luleå University of Technology, Sweden, with a diploma work in the ATLAS Collaboration at CERN, in 2001, and his \phd{} in Physics from Luleå University of Technology, Sweden, and the Swedish Graduate School of Space Technology in 2007.
He was an NFSR postdoc at IFPA in Liège 2008-2009.
Currently, he is a professor in Machine Learning at Luleå University of Technology, Sweden, where he works with brain-like computing and machine learning, and leads the effort in neuromorphic computing.
He was awarded the Gunnar Öquist Fellowship from the Kempe Foundations in 2014 and received a “New-Talents” award for original work in theoretical physics in 2004 from the International School of Subnuclear Physics in Erice.
\end{IEEEbiography}


%\vspace{-32pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/marcus_100x125.png}}]{Marcus~Liwicki}
received his M.S., degree in Computer Science from the Free University of Berlin, Germany, in 2004, his \phd{} degree from the University of Bern, Switzerland, in 2007, and his habilitation degree at the Technical University of Kaiserslautern, Germany, in 2011.
Currently, he is the chaired professor in Machine Learning and vice-rector for AI at Luleå University of Technology, Sweden.
His research interests include machine learning, pattern recognition, artificial intelligence, human-computer interaction, digital humanities, knowledge management, ubiquitous intuitive input devices, document analysis, and graph matching.
From October 2009 to March 2010 he visited Kyushu University (Fukuoka, Japan) as a research fellow (visiting professor), supported by the Japanese Society for the Promotion of Science.
In 2015, at the young age of 32, he received the ICDAR Young Investigator Award, a bi-annual award acknowledging outstanding achievements of in pattern recognition for researchers up to the age of 40.
\end{IEEEbiography}
